SSFlowNet: Semi-supervised Scene Flow Estimation On Point Clouds With Pseudo Label

In the domain of supervised scene flow estimation, the process of manual labeling is both time-intensive and financially demanding. This paper introduces SSFlowNet, a semi-supervised approach for scene flow estimation, that utilizes a blend of labeled and unlabeled data, optimizing the balance between the cost of labeling and the precision of model training. SSFlowNet stands out through its innovative use of pseudo-labels, mainly reducing the dependency on extensively labeled datasets while maintaining high model accuracy. The core of our model is its emphasis on the intricate geometric structures of point clouds, both locally and globally, coupled with a novel spatial memory feature. This feature is adept at learning the geometric relationships between points over sequential time frames. By identifying similarities between labeled and unlabeled points, SSFlowNet dynamically constructs a correlation matrix to evaluate scene flow dependencies at individual point level. Furthermore, the integration of a flow consistency module within SSFlowNet enhances its capability to consistently estimate flow, an essential aspect for analyzing dynamic scenes. Empirical results demonstrate that SSFlowNet surpasses existing methods in pseudo-label generation and shows adaptability across varying data volumes. Moreover, our semi-supervised training technique yields promising outcomes even with different smaller ratio labeled data, marking a substantial advancement in the field of scene flow estimation.

==> tool.tex <==
import matplotlib.pyplot as plt

# Data for plotting
models = ['3DFlowNet', 'Noisy-Pseudo', 'Ours(1/8)', 'Ours(1/16)', 'Ours(1/32)', 'Ours(1/64)']
epe = [0.028, 0.068, 0.010, 0.015, 0.026, 0.043]  # End Point Error (EPE)
as_metric = [0.929, 0.628, 0.976, 0.969, 0.942, 0.872]  # Accuracy under threshold (AS)
ar_metric = [0.981, 0.881, 0.991, 0.989, 0.973, 0.942]  # Accuracy Rate (AR)
out_metric = [0.146, 0.438, 0.028, 0.035, 0.074, 0.137]  # Outliers (Out)

# Creating line graphs
plt.figure(figsize=(10, 6))
plt.plot(models, epe, marker='o', label='EPE↓')
plt.plot(models, as_metric, marker='o', label='AS↑')
plt.plot(models, ar_metric, marker='o', label='AR↑')
plt.plot(models, out_metric, marker='o', label='Out↓')

# Adding title and labels
plt.title('Comparison of Scene Flow Estimation Models')
plt.xlabel('Models')
plt.ylabel('Metrics')
plt.xticks(rotation=45)
plt.legend()

# Displaying the plot
plt.tight_layout()
plt.show()

